Factorization in Call-by-Name and Call-by-Value Calculi via Linear Logic (long version)

In each variant of the lambda-calculus, factorization and normalization are two key-properties that show how results are computed. Instead of proving factorization/normalization for the call-by-name (CbN) and call-by-value (CbV) variants separately, we prove them only once, for the bang calculus (an extension of the lambda-calculus inspired by linear logic and subsuming CbN and CbV), and then we transfer the result via translations, obtaining factorization/normalization for CbN and CbV. The approach is robust: it still holds when extending the calculi with operators and extra rules to model some additional computational features.

==> 99-bangcalculus-translation.tex <==
\embedding*

\begin{proof}%\hfill
	%   Both proof are by induction on the $\lambda$-term $\Tm$.
	\begin{enumerate}
		\item \emph{Soundness:} We prove by induction on the $\lambda$-term $\LTm$ that if $\LTm \ToBeta \LTm'$ then $\Cbn{\LTm} \ToVal \Cbn{{\LTm'}}$ (this implies $\Cbn{\LTm} \ToTot \Cbn{{\LTm'}}$, since $\ToVal \,\subseteq\, \ToTot$). 
		According to the definition of $\LTm \ToBeta \LTm'$, there are the following cases:
		\begin{itemize}
			\item \emph{Root-step}, \Ie $\LTm \Defeq (\La{\var}{\LTmThree})\LTmTwo \Root{\beta} \LTmThree\Sub{\LTmTwo}{\var} \Eqdef {\LTm'}$: by \Reflemmap{substitution}{cbn}, %then 
			$\Cbn{\LTm} = \App{\La{\var}{\Cbn{\LTmThree}}}{\Bang{\Cbn{\LTmTwo}}} \allowbreak\Root{\ValScript} \Cbn{\LTmThree} \Sub{\Cbn{\LTmTwo}\!}{\var} = \Cbn{{\LTm'}}$.% (recall that $\WToVal \, \subseteq \, \ToVal$)
			
			\item  \emph{Abstraction}, \Ie $\LTm \Defeq \La{\var}{\LTmThree} \ToBeta \La{\var}{\LTmThree'} \Eqdef {\LTm'}$ with $\LTmThree \ToBeta \LTmThree'$: by %induction hypothesis
			\Ih, $\Cbn{\LTmThree} \ToVal \Cbn{{\LTmThree'}}$, thus $\Cbn{\LTm} = \La{\var}{\Cbn{\LTmThree}} \ToVal \La{\var}{\Cbn{{\LTmThree'}}} = \Cbn{{\LTm'}}$.
			
			\item \emph{Application left}, \Ie $\LTm \Defeq \LTmThree\LTmTwo \ToBeta \LTmThree'\LTmTwo \Eqdef {\LTm'}$ with $\LTmThree \ToBeta \LTmThree'$:
			analogous to the previous case.
%			by %induction hypothesis
%			\Ih $\Cbn{\LTmThree} \ToVal \Cbn{{\LTmThree'}}$\!, so $\Cbn{\LTm} = \App{\Cbn{\LTmThree}}{\Bang{{\Cbn{\LTmTwo}}}} \!\ToVal \App{\Cbn{{\LTmThree'}}}{\Bang{{\Cbn{\LTmTwo}}}} = \Cbn{{\LTm'}}$.
			
			\item \emph{Application right}, \Ie $\LTm \Defeq \LTmTwo\LTmThree \ToBeta \LTmTwo\LTmThree' \!\Eqdef \LTm'$ with $\LTmThree \ToBeta\! \LTmThree'$: 
			by %induction hypothesis, 
			\Ih $\Cbn{\LTmThree} \ToVal \Cbn{{\LTmThree'}}$\!, so $\Cbn{\LTm} = \App{\Cbn{\LTmTwo}}{\Bang{{\Cbn{\LTmThree}}}} \!\ToVal \App {\Cbn{\LTmTwo}} {\Bang{{\Cbn{{\LTmThree'}}}}} \!= \Cbn{{\LTm'}}$\!.
%			analogous to the previous case.
		\end{itemize}
		
		\emph{Completeness:} First, observe that $\Cbn{\LTm} \ToTot \TmTwo$ entails $\Cbn{\LTm} \ToVal \TmTwo$ since $\Der{\!}$ does not occur in $\Cbn{\LTm}$, hence $\Cbn{\LTm}$ is $\Derel$-normal.
		We prove by induction on the $\lambda$-term $\LTm$ that if $\Cbn{\LTm} \ToVal \TmTwo$ then $\TmTwo = \Cbn{{\LTm'}}$ and $\LTm \ToBeta \LTm'$ for some $\lambda$-term $\LTm'$. 
		According to the definition of $\Cbn{\LTm} \ToVal \TmTwo$, there are the following cases:
		\begin{itemize}
			\item \emph{Root-step}, \Ie $\Cbn{\LTm} \Defeq \App{\La{\var}{\Cbn{\LTmThree}}}{\Bang{\Cbn{\LTmFour}}} \allowbreak\Root{\ValScript} \Cbn{\LTmThree} \Sub{\Cbn{\LTmFour}}{\var} \Eqdef \TmTwo$: 
			by \Reflemmap{substitution}{cbn} $\TmTwo = \Cbn{(\LTmThree \Sub{\LTmFour}{\var})}$, so $\LTm = (\La{\var}{\LTmThree})\LTmFour \Root{\beta} \LTmThree\Sub{\LTmFour}{\var} \Eqdef {\LTm'}$ where $\Cbn{{\LTm'}} = \TmTwo$.
			
			\item  \emph{Abstraction}, \Ie $\Cbn{\LTm} \Defeq \La{\var}{\Cbn{\LTmThree}} \ToVal \La{\var}{\TmTwo'} \Eqdef \TmTwo$ with $\Cbn{\LTmThree} \ToVal \TmTwo'$: by %induction hypothesis
			\Ih, there is a $\lambda$-term $\LTmThree'$ such that $\Cbn{{\LTmThree'}} = \TmTwo'$ and $\LTmThree \ToBeta \LTmThree'$, thus $\LTm = \La{\var}{\LTmThree} \ToBeta \La{\var}{\LTmThree'} \Eqdef {\LTm'}$ where $\Cbn{{\LTm'}} = \La{\var}\Cbn{{\LTmThree'}} = \TmTwo$.
			
			\item \emph{Application left}, \Ie $\Cbn{\LTm} \Defeq \App{\Cbn{\LTmThree}}{\Bang{{\Cbn{\LTmFour}}}} \ToVal \App{\TmTwo'}{\Bang{{\Cbn{\LTmFour}}}} \Eqdef \TmTwo$ with $\Cbn{\LTmThree} \ToVal \TmTwo'$: 
%			analogous to the previous case.
			analogously to above.
			%       by induction hypothesis there is a $\lambda$-term $\TmThree'$ such that $\Cbn{{\TmThree'}} = \TmTwo'$ and $\TmThree \ToBeta \TmThree'$\!, so $\Tm = \TmThree\TmFour \ToBeta \TmThree'\TmFour \Eqdef {\Tm'}$ where $\Cbn{{\Tm'}} = \App{\Cbn{{\TmThree'}}}{\Bang{\Cbn{\TmFour}}} = \TmTwo$.
			
			\item \emph{Application right}, \Ie $\Cbn{\LTm} \!\Defeq \App{\Cbn{\LTmFour}}{\Bang{{\Cbn{\LTmThree}}}} \!\ToVal \App {\Cbn{\LTmFour}} \Bang{\TmTwo'} \!\Eqdef \TmTwo$ with $\Cbn{\LTmThree} \ToVal \TmTwo'$: by %induction hypothesis 
			\Ih, there is a $\lambda$-term $\LTmThree'$ such that $\Cbn{{\LTmThree'}} = \TmTwo'$ and $\LTmThree \ToBeta \LTmThree'$, so $\LTm = \LTmFour\LTmThree \ToBeta \LTmFour\LTmThree' \Eqdef \LTm'$ with $\Cbn{{\LTm'}} = \App{\Cbn{\LTmFour}}{\Bang{\Cbn{{\LTmThree'}}}} = \TmTwo$.
		\end{itemize}
		
		%     \item As $\WToTot$ is enough for the root-case in the proof of \Refpropp{embedding}{cbn}, 
		\item Since $\Root{\beta}$ is simulated by $\Root{\ValScript}$ and vice-versa (see the root-cases %in the proof of \Refpropp{embedding}{cbn}
		above), 
		\Refthmp{embedding}{cbn-head} is proved analogously to the proof of \Refthmp{embedding}{cbn} ($\WToVal$ replaces $\ToVal$, and $\WToBeta$ replaces $\ToBeta$), with the difference that, by definition, $\WToBeta$ and $\WToVal$ do not give rise to the case \emph{Application right}.
		%     (the only case non-preserving $\WToTot\!$ and $\WTot$, respectively, from the inductive hypothesis).
		%     Analogously to the proof of Prop.~\ref{prop:embedding}.\ref{prop:embedding.cbn}, with the difference that the $\beta^h$-reduction does not give rise to the case \emph{Application Right}.
		
		\item \emph{Soundness:} We prove by induction on the $\lambda$-term $\LTm$ that if $\LTm \ToBetav \LTm'$ then $\Cbv{\LTm} \ToDer\ToVal \Cbv{{\LTm'}}$.
		According to the definition of $\LTm \ToBetav \LTm'$, there are the following cases:
		\begin{itemize}
			\item \emph{Root-step}, \Ie $\LTm \Defeq (\La{\var}{\LTmThree})\LVal \Root{\Betav} \LTmThree\Sub{\LVal}{\var} \Eqdef \LTm'$ where $\LVal$ is a $\lambda$-value, \Ie a variable or an abstraction: then $\Cbv{\LVal} = \Bang{\TmTwo}$ for some $\TmTwo \in \BangSet$, hence $\Cbv{\LTm} = \App{\Der{\Bang{(\La{\var}{\Cbv{\LTmThree}})}}}{\Cbv{\LVal}} \allowbreak\WToDer\allowbreak \App{\La{\var}{\Cbv{\LTmThree}}}{\Cbv{\LVal}} \Root{\ValScript}\allowbreak \Cbv{\LTmThree} \Sub{\TmTwo}{\var} = \Cbv{{\LTm'}}$ by \Reflemmap{substitution}{cbv} (recall that $\WToDer \,\subseteq\,\ToDer$).
			
			\item  \emph{Abstraction}, \Ie $\LTm \Defeq \La{\var}{\LTmThree} \ToBetav \La{\var}{\LTmThree'} \Eqdef \LTm'$ with $\LTmThree \ToBetav \LTmThree'$: by %induction hypothesis
			\Ih, $\Cbv{\LTmThree} \ToDer\ToVal \Cbv{{\LTmThree'}}$; therefore $\Cbv{\LTm} = \Bang{(\La{\var}{\Cbv{\LTmThree}})} \ToDer\ToVal \Bang{(\La{\var}{\Cbv{{\LTmThree'}}})} = \Cbv{{\LTm'}}$.
			
			\item \emph{Application left}, \Ie $\LTm \Defeq \LTmThree\LTmTwo \ToBetav \LTmThree'\LTmTwo \Eqdef \LTm'$ with $\LTmThree \ToBetav \LTmThree'$: by %induction hypothesis
			\Ih $\Cbv{\LTmThree} \ToDer\ToVal \Cbv{{\LTmThree'}}$; therefore $\Cbv{\LTm} = \App{\Der{\Cbv{\LTmThree}}}{{\Cbv{\LTmTwo}}} \ToDer\ToVal \App{\Der{\Cbv{{\LTmThree'}}}}{{\Cbv{\LTmTwo}}} = \Cbv{{\Tm'}}$.
			
			\item \emph{Application right}, \Ie $\LTm \Defeq \LTmTwo\LTmThree \ToBetav \LTmTwo\LTmThree' \!\Eqdef \LTm'$ with $\LTmThree \ToBetav\! \LTmThree'$: 
			analogous to the previous case.
			%       by induction hypothesis, $\Cbv{\TmThree} \ToTot^2 \Cbv{{\TmThree'}}$\!, therefore 
			%       $\Cbv{\Tm} = \App{\La{\varTwo}\App{\varTwo}{{\Cbv{\TmThree}}}}{\Cbv{\TmFour}} \ToTot^2 \App{\La{\varTwo}\App{\varTwo}{{\Cbv{{\TmThree'}}}}}{\Cbv{\TmFour}} = \Cbv{{\Tm'}}$.
		\end{itemize}
		
		\emph{Completeness:} 
		%     As an initial remark, it is immediate to prove by straightforward induction on the $\lambda$-term $\Tm$ that $\Cbv{\Tm}$ is $\ValScript$-normal, so the fact that $\Cbv{\Tm} \ToBang \TmTwo_0 \ToVal \TmTwo$ implies that the only $\ValScript$-redex in $\TmTwo_0$ has been created by reducing the $\Derel$-redex in $\Cbv{\Tm} \ToBang \TmTwo_0$ and is absent in $\Cbv{{\Tm}}$.
		We prove by induction on $\TmTwo_0 \in \BangSet$ that if $\Cbv{\LTm} \ToDer \TmTwo_0 \ToVal \TmTwo$ then $\TmTwo = \Cbv{{\LTm'}}$ and $\LTm \ToBetav \LTm'$ for some $\lambda$-term $\LTm'$.
		According to the definition of $\TmTwo_0 \ToVal \TmTwo$, there are the following cases:
		\begin{itemize}
			\item \emph{Root-step}, \Ie $\TmTwo_0 \Defeq \App{\La{\var}{\TmThree}}{\Bang{\TmFour}} \Root{\ValScript} \TmThree\Sub{\TmFour}{\var} \Eqdef \TmTwo$.
			By \Refrmk{cbv-val-normal}, necessarily $\Cbv{\LTm} = \App{\Der{\Bang{(\La{\var}{\TmThree})}}}{\Bang{\TmFour}}$ and hence $\LTm = (\La{\var}{\LTmThree_0})\LVal$ for some $\lambda$-term $\LTmThree_0$ and some $\lambda$-value $\LVal$ such that $\Cbv{\LTmThree_0} = \TmThree$ and $\Cbv{\LVal} = \Bang{\TmFour}$.
			Note that $\Cbv{\LTm} \WToDer \TmTwo_0$. 
			Let $\LTm' \Defeq \LTmThree_0 \Sub{\LVal}{\var}$: then, $\LTm \Root{\Betav} \LTm'$ and $\Cbv{{\LTm'}} = \Cbv{\LTmThree_0} \Sub{\TmFour}{\var} = \TmTwo$ by \Reflemmap{substitution}{cbv}.
			
			\item \emph{Abstraction}, \Ie $\TmTwo_0 \Defeq \La{\var}{\TmThree_0} \ToVal \La{\var}{\TmThree'} \Eqdef \TmTwo$ with $\TmThree_0 \ToVal \TmThree'$.
			This case is impossible because, according to \Refrmk{cbv-val-normal}, necessarily $\Cbv{\LTm} = \La{\var}{\TmThree}$ for some $\ValScript$-normal $\TmThree \in \BangSet$ such that $\TmThree \ToDer \TmThree_0$, but there is no $\lambda$-term $\LTm$ such that $\Cbv{\LTm}$ is an abstraction.
			\item \emph{Dereliction}, \Ie $\TmTwo_0 \Defeq \Der{\TmThree_0} \ToVal \Der{\TmThree'} \Eqdef \TmTwo$ with $\TmThree_0 \ToVal \TmThree'$.
			This case is impossible because, according to \Refrmk{cbv-val-normal}, necessarily $\Cbv{\LTm} = \Der{\TmThree}$  for some $\ValScript$-normal $\TmThree \in \BangSet$ such that $\TmThree \ToDer \TmThree_0$, but there is no $\lambda$-term $\LTm$ such that $\Cbv{\LTm}$ is a dereliction.
			
			\item \emph{Application left}, \Ie $\TmTwo_0 \Defeq \App{\TmThree_0}{\TmThree_1} \ToVal \App{\TmThree'}{\TmThree_1} \Eqdef \TmTwo$ with $\TmThree_0 \ToVal \TmThree'$.
			%According to 
			By \Refrmk{cbv-val-normal}, %necessarily 
			$\Cbv{\LTm} = \App{\Der{\TmFive}}{\TmThree_1}$ for some $\ValScript$-normal $\TmFive \in \BangSet$ such that $\Der{\TmFive} \ToDer \TmThree_0$, and thus $\TmThree_0 = \Der{\TmFive_0}$ where $\TmFive \ToDer \TmFive_0$ (indeed $\TmFive = \Bang{\TmThree_0}$ is impossible because $\TmFive$ is $\ValScript$-normal), and hence $\TmThree' = \Der{\TmFive'}$ with $\TmFive_0 \ToVal \TmFive'$.
			So, $\LTm = \LTmFour\LTmFour_1$ for some $\lambda$-terms $\LTmFour$ and $\LTmFour_1$ such that $\Cbv{\LTmFour} = \TmFive$ and $\Cbv{\LTmFour_1} = \TmThree_1$ with $\Cbv{\LTmFour} \ToDer \TmFive_0 \ToVal \TmFive'$.
			By %induction hypothesis, 
			\Ih, $\TmFive' = \Cbv{{\LTmFour'}}$ and $\LTmFour \ToBetav \LTmFour'$ for some $\lambda$-term $\LTmFour'$.
			Let $\LTm' \Defeq \LTmFour'\LTmFour_1$: then, $\LTm = \LTmFour\LTmFour_1 \ToBetav %\TmFour'\TmFour = 
			\LTm'$ and $\Cbv{{\LTm'}} = \App{\Der{\Cbv{{\LTmFour'}}}}{\Cbv{\LTmFour_1}} = \TmTwo$.
			
			\item \emph{Application right}, \Ie $\TmTwo_0 \Defeq \App{\TmThree_1}{\TmThree_0} \ToVal \App{\TmThree_1}{\TmThree'} \Eqdef \TmTwo$ with $\TmThree_0 \ToVal \TmThree'$.
			%According to
			By \Refrmk{cbv-val-normal}, necessarily $\Cbv{\LTm} = \App{\Der{\TmFive_1}}{\TmThree}$ for some $\ValScript$-normal $\TmThree, \TmFive_1 \in \BangSet$ such that $\Der{\TmFive_1} = \TmThree_1$ and $\TmThree \ToDer \TmThree_0$.
			So, $\LTm = \LTmFour_1\LTmFour$ for some $\lambda$-terms $\LTmFour_1$ and $\LTmFour$ such that $\Cbv{\LTmFour_1} = \TmFive_1$ and $\Cbv{\LTmFour} = \TmThree$ with $\Cbv{\LTmFour} \ToDer \TmThree_0 \ToVal \TmThree'$.
			By %induction hypothesis,
			\Ih, $\TmThree' = \Cbv{{\LTmFour'}}$ and $\LTmFour \ToBetav \LTmFour'$ for some $\lambda$-term $\LTmFour'$.
			Let $\LTm' \Defeq \LTmFour_1\LTmFour'$: then, $\LTm = \LTmFour_1\LTmFour \ToBetav %\TmFour'\TmFour = 
			\LTm'$ and $\Cbv{{\LTm'}} = \App{\Der{\Cbv{\LTmFour_1}}}{\Cbv{{\LTmFour'}}} = \TmTwo$.
			
			\item \emph{Box}, \Ie $\TmTwo_0 \Defeq \Bang{\TmThree_0} \ToVal \Bang{\TmThree'} \Eqdef \TmTwo$ with $\TmThree_0 \ToVal \TmThree'$.
			According to \Refrmk{cbv-val-normal}, necessarily $\Cbv{\LTm} = \Bang{\TmThree}$ for some $\ValScript$-normal $\TmThree \in \BangSet$ such that $\TmThree \ToDer \TmThree_0$.
			So, $\LTm = \La{\var}{\LTmFour}$ (since $\Cbv{\LTm}$ is a box and $\Cbv{\var}$ is $\Derel$-normal) for some $\lambda$-term $\LTmFour$ such that $\TmThree = \La{\var}\Cbv{\LTmFour}$, and hence there are $\TmFive_0, \TmFive' \in \BangSet$ such that $\TmThree_0 = \La{\var}{\TmFive_0}$ and $\TmThree' = \La{\var}{\TmFive'}$  with $\Cbv{\LTmFour} \ToDer \TmFive_0 \ToVal \TmFive'$.
			By %induction hypothesis, 
			\Ih, $\TmFive' = \Cbv{{\LTmFour'}}$ and $\LTmFour \ToBetav \LTmFour'$ for some $\lambda$-term $\LTmFour'$.
			Let $\LTm' \Defeq \La{\var}{\LTmFour'}$: then, $\LTm = \La{\var}{\LTmFour} \ToBetav %\La{\var}{\TmFour'} = 
			\LTm'$ and $\Cbv{{\LTm'}} = \Bangp{\La{\var}{\Cbv{{\LTmFour'}}}} = \TmTwo$.
		\end{itemize}
		
		\item Since $\Root{\Betav}$ is simulated by $\WToDer\Root{\ValScript}$ and vice-versa (see the root-cases %in the proof of \Refpropp{embedding}{cbv}
		above), \Refthmp{embedding}{cbv-head} is proved analogously to the proof of \Refthmp{embedding}{cbv} (replace $\ToVal$ with $\WToVal$, and $\ToDer$ with $\WToDer$, as well as $\ToBetav$ with $\WToBetav$), with the difference that $\WToBetav$ does not give rise to the case \emph{Abstraction} (in the soundness proof) and \emph{Box} (in the completeness proof). 
		%     (the only case non-preserving $\WToTot\!$ from the inductive hypothesis).
		\qedhere
		%     , which is replaced by the following case:
		%     \begin{itemize}
		%       \item \emph{Inside a $\beta$-like redex}, \Ie $\Tm \Defeq (\La{\var}{\TmTwo})\TmThree \WToBetav (\La{\var}{\TmTwo'})\TmThree \Eqdef \Tm'$ with $\TmTwo \WToBetav \TmTwo'$:
		%       by induction hypothesis, $\Cbv{\TmTwo} \WToTot\WToTot \Cbv{{\TmTwo'}}$ and therefore $\Cbv{\Tm} = \App{\Der{\Bang{(\La{\var}\Cbv{\TmTwo})}}}{\Cbv{\TmThree}} \ToTot\ToTot \App{\La{\varTwo}{\App{\varTwo}{\Cbv{\TmThree}}}}{\Bang{(\La{\var}\Cbv{{\TmTwo'}})}} = \Cbv{{\Tm'}}$.
		%       \qedhere
		%       FALSE! It works taking the normal forms of $\ToBang$
		%     \end{itemize}
	\end{enumerate}
\end{proof}


==> fig-bangcalculus.tex <==
\begin{figure}[!t]
  \centering
  \scalebox{0.8}{\parbox{1.05\linewidth}{
  \begin{align*}
    \text{\emph{Terms}:}		&& \Tm, \TmTwo &\Coloneqq \, \var  \,\mid\, \La{\var}\Tm \,\mid\, \App{\Tm}{\TmTwo} \,\mid\, \Der{\Tm}	\,\mid \, \Bang{\Tm}			&&(\textup{set: } \BangSet)  \\
    \text{\emph{Contexts}:}	&& \Ctx			&\Coloneqq \, \Hole{\cdot} \mid \La{\var}{\Ctx} \mid \App{\Ctx}{\Tm} \mid \App{\Tm}{\Ctx} \mid \Der{\Ctx} \mid \Bang{\Ctx}	&&(\textup{set: }\CtxSet) \\
    \text{\emph{\Ground\ contexts}:}&&\WCtx  		&\Coloneqq \, \Hole{\cdot} \mid \La{\var}{\WCtx} \mid \App{\WCtx}{\Tm} \mid \App{\Tm}{\WCtx}  \mid \Der{\WCtx} 			&&(\textup{set: }\WCtxSet)	     
  \end{align*}
  \begin{align*}
    \text{\emph{Root-steps}:}	&& \App{\La{\var}{\Tm}}{\ValTwo} &\Root{\ValScript} \Tm\Sub{\TmTwo}{\var}  \quad \Derp{\Bang{\Tm}} \Root{\Derel} \Tm \quad \Root{\Tot} \, \Defeq \ \Root{\ValScript} \cup \Root{\Derel} \\[.2\baselineskip]
    \Rule\text{-\emph{reduction}:} &&   \Tm \To{\Rule}  \TmTwo \ &\Leftrightarrow \ \exists \, \Ctx \in \CtxSet, \, \exists\, \Tm'\!, \TmTwo' \!\in \BangSet : \Tm = \Ctxp{\Tm'}, \, \TmTwo = \Ctxp{\TmTwo'}, \, \Tm' \!\Root{\Rule} \TmTwo' \\
    \Weak{\Rule}\text{-\emph{reduction}:} &&   \Tm \WTo{\Rule}  \TmTwo \ &\Leftrightarrow \ \exists \, \WCtx \in \WCtxSet, \,\exists\, \Tm'\!, \TmTwo' \!\in \BangSet : \Tm = \WCtxp{\Tm'}, \, \TmTwo = \WCtxp{\TmTwo'}, \, \Tm' \!\Root{\Rule} \TmTwo'
%    \\[-1.5\baselineskip]
  \end{align*}
  }}
  \caption{The bang calculus: its syntax and reduction rules, where $\Rule \in \{\ValScript, \Derel, \Tot\}$.}
  \label{fig-bangcalculus}
\end{figure}


==> fig-bangcalculusNew.tex <==
\begin{figure}[!t]
  \centering
  \scalebox{0.85}{\parbox{1.05\linewidth}{
  \begin{align*}
    \text{\emph{Terms}:}		&& \Tm, \TmTwo &\Coloneqq \, \var  \,\mid\, \La{\var}\Tm \,\mid\, \App{\Tm}{\TmTwo}	\,\mid \, \Bang{\Tm}			&&(\textup{set: } \BangSet)  \\
    \text{\emph{Contexts}:}	&& \Ctx			&\Coloneqq \, \Hole{\cdot} \mid \La{\var}{\Ctx} \mid \App{\Ctx}{\Tm} \mid \App{\Tm}{\Ctx} \mid  \Bang{\Ctx}	&&(\textup{set: }\CtxSet) 
%    \\
%    \text{\emph{\Ground\ contexts}:}&&\WCtx  		&\Coloneqq \, \Hole{\cdot} \mid \La{\var}{\WCtx} \mid \App{\WCtx}{\Tm} \mid \App{\Tm}{\WCtx} 		&&(\textup{set: }\WCtxSet)	     
  \end{align*}
  \begin{align*}
%    \text{\emph{Root-steps}:}	&& \App{\La{\var}{\Tm}}{\ValTwo} &\Root{\ValScript} \Tm\Sub{\TmTwo}{\var}  \quad \Derp{\Bang{\Tm}} \Root{\Derel} \Tm \quad \Root{\Tot} \, \Defeq \ \Root{\ValScript} \cup \Root{\Derel}
    \text{\emph{Root-step}:}	&& \App{\La{\var}{\Tm}}{\ValTwo} &\Root{\Tot} \Tm\Sub{\TmTwo}{\var}  
    \\ %[.2\baselineskip]
    \Tot\text{-\emph{reduction}:} &&   \Tm \To{\Rule}  \TmTwo \ &\Leftrightarrow \ \exists \, \Ctx \in \CtxSet, \, \exists\, \Tm'\!, \TmTwo' \!\in \BangSet : \Tm = \Ctxp{\Tm'}, \, \TmTwo = \Ctxp{\TmTwo'}, \, \Tm' \!\Root{\Rule} \TmTwo' 
%    \\
%    \Weak{\Rule}\text{-\emph{reduction}:} &&   \Tm \WTo{\Rule}  \TmTwo \ &\Leftrightarrow \ \exists \, \WCtx \in \WCtxSet, \,\exists\, \Tm'\!, \TmTwo' \!\in \BangSet : \Tm = \WCtxp{\Tm'}, \, \TmTwo = \WCtxp{\TmTwo'}, \, \Tm' \!\Root{\Rule} \TmTwo'
%    \\[-1.5\baselineskip]
  \end{align*}
  }}
  \caption{The bang calculus: its syntax and reduction rule.}
  \label{fig-bangcalculus}
\end{figure}


==> fig-lambdacalculus.tex <==
\begin{figure}[!t]
  \centering
%  \scaalebox{0.9}{\parbox{1.067\linewidth}{
  \begin{align*}
    \lambda\text{-\emph{terms}:}		&& \LTm, \LTmTwo, \LTmThree &\Coloneqq \, \LVal  \,\mid\,  \LTm\LTmTwo			&&(\textup{set: } \Lambda)  \\
    \lambda\text{-\emph{values}:}		&& \LVal &\Coloneqq \, \var  \,\mid\, \La{\var\,}\LTm 					&&(\textup{set: } \LambdaVal)  \\
    \lambda\text{-\emph{contexts}:}	&& \LCtx		&\Coloneqq \, \Hole{\cdot} \mid \La{\var}{\LCtx} \mid \LCtx\LTm \mid \LTm\LCtx 	&&(\textup{set: }\LambdaOpCtx) \\
    \text{\emph{\CbN\ \ground\ $\lambda$-contexts}:}&&\NCtx	&\Coloneqq \, \Hole{\cdot} \mid \La{\var}{\NCtx} \mid \NCtx\LTm 	&&(\textup{set: }\Lambda_\NCtx)	     \\
    \text{\emph{\CbV\ \ground\ $\lambda$-contexts}:}&&\VCtx	&\Coloneqq \, \Hole{\cdot} \mid \VCtx\LTm \mid \LTm\VCtx  		&&(\textup{set: }\Lambda_\VCtx)	     
%    \\[-2\baselineskip]
  \end{align*}
  \begin{align*}
    \text{\emph{Root-steps}:}	&& (\La{\var}{\LTm}){\TmTwo} &\Root{\beta} \LTm\Sub{\TmTwo}{\var} \ (\text{\CbN})  \qquad (\La{\var}{\LTm}){\LVal} \Root{\Betav} \LTm\Sub{\LVal}{\var} \ (\text{\CbV}) \\[.2\baselineskip]
    \Rule\text{-\emph{reduction}:} &&   \LTm \To{\Rule}  \LTmTwo \ &\Leftrightarrow \ \exists \, \Ctx \in \Lambda_\Ctx, \, \exists\, \LTm'\!, \LTmTwo' \!\in \Lambda : \LTm = \Ctxp{\LTm'}, \, \LTmTwo = \Ctxp{\LTmTwo'}, \, \LTm' \!\Root{\Rule} \LTmTwo' 
%    \\
%    \Weak{\beta}\text{-\emph{reduction}:} &&   \LTm \WToBeta  \LTmTwo \ &\Leftrightarrow \ \exists \, \NCtx \in \Lambda_\NCtx, \,\exists\, \LTm'\!, \LTmTwo' \!\in \Lambda : \LTm = \NCtxp{\LTm'}, \, \LTmTwo = \NCtxp{\LTmTwo'}, \, \LTm' \!\Root{\beta} \LTmTwo' 
%    \\
%    \Weak{\Betav}\text{-\emph{reduction}:} &&   \LTm \WToBetav  \LTmTwo \ &\Leftrightarrow \ \exists \, \VCtx \in \Lambda_\VCtx, \,\exists\, \LTm'\!, \LTmTwo' \!\in \Lambda : \LTm = \VCtxp{\LTm'}, \, \LTmTwo = \VCtxp{\LTmTwo'}, \, \LTm' \!\Root{\Betav} \LTmTwo'
%    \\[-1.5\baselineskip]
  \end{align*}
%  }}
  \caption{The \CbN\ and \CbV\ $\lambda$-calculi: their syntax and reduction, with $\Rule \in \{\beta, \Betav\}$.}
  \label{fig-lambdacalculus}
\end{figure}


==> fig-parallel.tex <==
\begin{figure}[!bt]
  \centering
  \scalebox{0.85}{
    \begin{prooftree}[label separation=0.3em]
      \infer0[\footnotesize$\mathsf{var}$]{\Var \ParallelVal \Var}
    \end{prooftree}
    \quad
    \begin{prooftree}[label separation=0.3em]
      \hypo{\Tm \ParallelVal \TmTwo}
      \infer1[\footnotesize$\mathsf{\lambda}$]{\lambda\Var\,\Tm \ParallelVal \lambda\Var\,\TmTwo}
    \end{prooftree}
    \quad
    \begin{prooftree}[label separation=0.3em]
      \hypo{\Tm \ParallelVal \TmTwo}
      \infer1[\footnotesize$\oc$]{\Bang{\Tm} \ParallelVal \Bang{\TmTwo}}
    \end{prooftree}
    \quad
    \begin{prooftree}[label separation=0.3em]
      \hypo{\Tm \ParallelVal \TmTwo}
      \infer1[\footnotesize$\Der{\!}$]{\Der{\Tm} \ParallelVal \Der{\TmTwo}}
    \end{prooftree}
%   }
%   \scalebox{0.85}{
    \quad
    \begin{prooftree}[separation=1.2em, label separation=0.3em]
      \hypo{\Tm \ParallelVal \TmTwo}
      \hypo{\TmThree \ParallelVal \TmFour}
      \infer2[\footnotesize$@$]{\App{\Tm}{\TmThree} \ParallelVal \App{\TmTwo}{\TmFour}}
    \end{prooftree}
    \quad
    \begin{prooftree}[separation=1.3em, label separation=0.3em]
      \hypo{\Tm \ParallelVal \TmTwo}
      \hypo{\TmThree \ParallelVal \TmFour}
      \infer2[\footnotesize$\ValScript$]{\App{\La{\Var}{\Tm}}{\ValThree} \ParallelVal \TmTwo\Sub{\TmFour}{\Var}}
    \end{prooftree}
  }
  \caption{Parallel $\ValScript$-reduction.}
  \label{fig:parallel}
\end{figure}

